On the Compression of Recurrent Neural Networks with an Application to LVCSR acoustic modeling for Embedded Speech Recognition

We study the problem of compressing recurrent neural networks (RNNs). In particular, we focus on the compression of RNN acoustic models, which are motivated by the goal of building compact and accurate speech recognition systems which can be run efficiently on mobile devices. In this work, we present a technique for general recurrent model compression that jointly compresses both recurrent and non-recurrent inter-layer weight matrices. We find that the proposed technique allows us to reduce the size of our Long Short-Term Memory (LSTM) acoustic model to a third of its original size with negligible loss in accuracy.

==> hashnets.tex <==
% !TEX root = lstm_model_compression.tex
As an alternative to the proposed compression approach, we also consider the
use of HashNets~\cite{ChenWilsonTyreeEtAl15}, which have been proposed
recently. The main idea behind HashNets is to impose a form of parameter tying
over the individual weight matrices of the network based on the use of a set of
hash functions. More precisely, let $W \in \R^{m \times n}$ represent one of
the weight matrices in the network, which is to be represented in terms of a
smaller number of parameters $k \ll mn$. If we denote by $\N_{i}$ the set of
natural numbers between $1$ and $i$, then we define a hash function $\xi:
\N_{m} \times \N_{n} \to \N_{k}$ which maps each pair of indices $(i, j)$ into
one of $k$ values. Thus, the hash function defines the parameter tying in the
weight matrix, since the elements $W_{i, j}$ and $W_{i', j'}$ are tied together
if $\xi(i, j) = \xi(i', j')$. The hash function $\xi$ corresponding to a
particular weight matrix is held fixed throughout the training process. Thus,
to summarize the `virtual' weight matrix $W$ of mn elements is represented in
terms of $k$ real weights $W_{i, j} = w_{\xi(i, j)}$.

\textbf{Tony, can you please read and verify that this is correct?}
In order to directly compare HashNets to the proposed SVD based compression,
our implementation of HashNets uses a separate hash function for each of the
recurrent and inter-layer weight matrices. Given a baseline model, we
initialize the `real' weights $w_{1}, \cdots, w_{k}$ as the mean of all weights
that are hashed into a particular bucket, \begin{equation}
w_{r} = \frac {\sum_{(i, j) \text{ s. t. } \xi{(i, j) = r}} W_{i, j}} {\sum_{(i, j) \text{ s. t. } \xi{(i, j) = r}} 1}
\end{equation}

Following this initialization, the weight matrices are then further fine-tuned
by training the neural network by backpropagation, during which we enforce the
parameter tying determined by the hash function.


==> lstm.tex <==
This section describes LSTMs and CTC training

